Gliding on ice in search of accurate and cost-effective computational methods for astrochemistry on grains: the puzzling case of the HCN isomerization

The isomerization of hydrogen cyanide to hydrogen isocyanide on icy grain surfaces is investigated by an accurate composite method (jun-Cheap) rooted in the coupled cluster ansatz and by density functional approaches. After benchmarking density functional predictions of both geometries and reaction energies against jun-Cheap results for the relatively small model system HCN -- (H2O)2 the best performing DFT methods are selected. A large cluster containing 20 water molecules is then employed within a QM/QM$'$ approach to include a realistic environment mimicking the surface of icy grains. Our results indicate that four water molecules are directly involved in a proton relay mechanism, which strongly reduces the activation energy with respect to the direct hydrogen transfer occurring in the isolated molecule. Further extension of the size of the cluster up to 192 water molecules in the framework of a three-layer QM/QM'/MM model has a negligible effect on the energy barrier ruling the isomerization. Computation of reaction rates by transition state theory indicates that on icy surfaces the isomerization of HNC to HCN could occur quite easily even at low temperatures thanks to the reduced activation energy that can be effectively overcome by tunneling.

==> cut.tex <==





Gardebien et al. proposed cyclic complexes for both reactants and products, i. e. HCN\ce{(H2O)2} and HNC\ce{(H2O)2}. Moreover, they identified a possible linear complex for the product isoenergetic to the cyclic one. However, since we are not interested in a full characterization of the PES, just the cyclic structure will be considered. 

To be sure that this was a safe choice, we tested the energy of both structures at DFT level: in the majority of cases the acyclic structure collapsed to the cyclic one, we managed to optimize both the structures at BMK-D3(BJ)/aug-cc-pVTZ level and the cyclic configuration is stabler than the linear one. 

In this paper, we present this analysis for both geometry and energy and suggest the functional/basis combinations with the best trade-off between accuracy and computational cost for interstellar ice analogues simulations.




With this strategy we can select the suitable functional/basis combination with the optimal accuracy/cost trade-off for both accurate geometries and energies when reactivity on water ice comes into play. 

Removed from the test because of the new table 1:

\textcolor{red}{Electronic energies were corrected for harmonic zero-Point vibrational energies (ZPVE) evaluated at the rev-DSDPBEP86-D3/jul-cc-pVTZ level of theory. BSSE????!!\cite{Boys&Bernard-1970,Simon-BSSE-1996}}  
We used CFOUR\cite{Stanton-2020-CFOUR} package for geometry optimizations at CCSD(T) level and the GAUSSIAN16\cite{g16} software for all the remaining calculations.




Things to check:

POINT 1: Table 1 no ZPE corrections --> Done
POINT 2: Statistical analysis for energy (is ZPE included? check) --> ZPE is not included, anyways since I added the same ZPE to all of the values the errors should be the same. Right? --> Done
POINT 3: Koch values comparison. I put in a Table jChS and ONIOM results and compared to Koch et al. values. Don't know if and which include in the text. If you take a look and tell me what you think I can make changes in the main.tex. Note here values are in kcal/mol as in Koch et al. but if you what to put them in the text I can convert            everything to kJ/mol which is what we have used so far.

\begin{table}[]

\caption{Formation energies calculated with respect to HNC-(H$_{2}$O)$_{2}$ as in Koch et al. jChS, ONIOM both with and without ZPE and Koch et al. values for HNC-(H$_{2}$O)$_{3}$(H$_{2}$O)$_{7}$. Results are in kcal/mol.}
\label{table:Formation_ene-Koch} 
\begin{tabular}{lcccc}
\hline
                      & \textbf{HNC-(H\boldmath{$_{2}$}O)\boldmath{$_{2}$}} & \textbf{TS} & \textbf{HCN-(H\boldmath{$_{2}$}O)$_{2}$}  \\
\hline

\textbf{jChS} & 0 & 20.2 & -11.6\\
\textbf{ONIOM} & 0 & 11.8 & -10.4\\
\textbf{ONIOM with ONIOM ZPE} & 0 & 7.7 & -10.4\\
\textbf{Koch et al.} & 0 & 3.3 & -9.9
\\
\hline
\end{tabular}
\end{table}


            
POINT 4: Have jChS and ONIOM in Fig. 5? No they don't --> Done


POINT 5: (-) in Figure PES. --> Fixed
POINT 6: y axis DeltaE --> Done

POINT 7: BSSE value at rDSD
        BSSE values at rDSDPBEP86-julTZ in kJ/mol here the dimer is considered as single fragment and no values are available for the TS:
        HCN-(H2O)2 => 1.31
        HNC-(H2O)2 => 1.90
        
        BSSE values at rDSDPBEP86-julTZ in kJ/mol here the dimer is considered made of two fragments and no values are available for the TS:
        (H2O)2 => 0.96
        HCN-(H2O)2 => 2.29
        HNC-(H2O)2 => 2.91
        
        gCP evaluated with Grimme programm at DFT/def2-TZVP in kJ/mol:
        HCN => 2.14
        HNC => 2.25
        (H2O)2 => 10.45
        HCN-(H2O)2 => 14.38
        TS => 19.30
        HNC-(H2O)2 => 15.50 
        

        
        
        
        
        

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
